Prompt Optimization Meets Subspace Representation Learning for Few-shot Out-of-Distribution Detection

The reliability of artificial intelligence (AI) systems in open-world settings depends heavily on their ability to flag out-of-distribution (OOD) inputs unseen during training. Recent advances in large-scale vision-language models (VLMs) have enabled promising few-shot OOD detection frameworks using only a handful of in-distribution (ID) samples. However, existing prompt learning-based OOD methods rely solely on softmax probabilities, overlooking the rich discriminative potential of the feature embeddings learned by VLMs trained on millions of samples. To address this limitation, we propose a novel context optimization (CoOp)-based framework that integrates subspace representation learning with prompt tuning. Our approach improves ID-OOD separability by projecting the ID features into a subspace spanned by prompt vectors, while projecting ID-irrelevant features into an orthogonal null space. To train such OOD detection framework, we design an easy-to-handle end-to-end learning criterion that ensures strong OOD detection performance as well as high ID classification accuracy. Experiments on real-world datasets showcase the effectiveness of our approach.

==> iclr2026/def.tex <==


\newcommand{\Y}{\boldsymbol{Y}}
\newcommand{\G}{\boldsymbol{G}}
%\newcommand{\D}{\boldsymbol{D}}
\newcommand{\Q}{\boldsymbol{Q}}
\newcommand{\C}{\boldsymbol{C}}
\newcommand{\U}{\boldsymbol{U}}
\newcommand{\F}{\boldsymbol{F}}
\newcommand{\K}{\mathcal{K}}
\newcommand{\one}{\boldsymbol{1}}
\renewcommand{\H}{\boldsymbol{H}}
\newcommand{\M}{\boldsymbol{M}}
\newcommand{\A}{\boldsymbol{A}}
\newcommand{\B}{\boldsymbol{B}}
\renewcommand{\S}{\boldsymbol{S}}
\newcommand{\Z}{\boldsymbol{Z}}

\newcommand{\p}{\boldsymbol{p}}
\newcommand{\z}{\boldsymbol{z}}
\renewcommand{\c}{\boldsymbol{c}}
\newcommand{\y}{\boldsymbol{y}}
\renewcommand{\v}{\boldsymbol{v}}
\renewcommand{\u}{\boldsymbol{u}}
\newcommand{\w}{\boldsymbol{w}}
\newcommand{\q}{\boldsymbol{q}}
\renewcommand{\b}{\boldsymbol{b}}
\newcommand{\m}{\boldsymbol{m}}
\renewcommand{\a}{\boldsymbol{a}}
\renewcommand{\th}{\boldsymbol{\theta}}
\newcommand{\cone}[1]{\textsf{cone}\left\{#1\right\}}
\newcommand{\conv}[1]{\textsf{conv}\left\{#1\right\}}
%\DeclareMathOperator*{\argmin}{\arg\min}
\newcommand{\bOmega}{\bm{\varOmega}}
\newcommand{\bTheta}{\bm{\varTheta}}
\newcommand{\bL}{\bm{\varPsi}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bC}{\bm{C}}
\newcommand{\bPi}{\bm{\varPi}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bS}{\bm{S}}
\newcommand{\bG}{\bm{G}}
\newcommand{\bXi}{\bm{\varXi}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bi}{\bm{i}}
\newcommand{\bZ}{\bm{Z}}
\newcommand{\bQ}{\bm{Q}}

\newcommand{\bg}{\bm{g}}
\newcommand{\bp}{\bm{p}}
\newcommand{\bmu}{\bm{\mu}}
\newcommand{\bnu}{\bm{\nu}}
\newcommand{\bpsi}{\bm{\psi}}

\newcommand{\bbR}{\mathbb{R}}

\newcommand{\cC}{\mathcal{C}}
\newcommand{\cO}{\mathcal{O}}


\newcommand{\ones}{\bm{\mathit{1}}}

% \DeclareMathOperator*{\minimize}{\textrm{minimize}}
% \DeclareMathOperator{\rank}{rank}
% \DeclareMathOperator{\tr}{Tr}

% \DeclareMathOperator{\prob}{{\sf Pr}}
% \DeclareMathOperator{\Expect}{\mathbb{E}}

\newtheorem{lemma}{Lemma}
\newtheorem{Prop}{Proposition}
\newtheorem{Theorem}{Theorem}
\newtheorem{Def}{Definition}
\newtheorem{Assump}{Assumption}
\newtheorem{Corollary}{Corollary}
\newtheorem{Property}{Property}
\newtheorem{Observation}{Observation}
\newtheorem{Exa}{Example}
\newtheorem{Remark}{Remark}
\newtheorem{Fact}{Fact}

%--- define color
%\definecolor{orange}{RGB}{255,107,0}
\def\blue{\color{blue}}
\def\red{\color{red}}
\def\orange{\color{orange}}
\def\green{\color{green}}
\def\purple{\color{purple}}

==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/name.tex <==
  
\begin{center}
    {\bf Supplementary Material of ``Prompt Optimization Meets Subspace Representation Learning for Few-shot Out-of-Distribution Detection''}
\end{center}


 	%$\bm \varDelta_K = \{\bm x \in \mathbb{R}^K : \sum_i \bm x(i) =1, \bm x \ge \bm 0\}$ denotes the probability simplex. 
  %$\bm X \ge \bm 0$ implies that all the entries of the matrix $\bm X$ are nonnegative. 
  %$\mathbb{I}[A]$ denotes an indicator function for the event $A$ such that $\mathbb{I}[A]=1$ if the event $A$ happens, otherwise $\mathbb{I}[A]=0$. ${\sf CE}(\bm x,y) = -\sum_{k=1}^K \mathbb{I}[{y}=k]\log(\bm x(k))$ denotes the cross entropy function. 
  \section{Related Works}
%{\red need some refinement}
\textbf{OOD Detection}.
Traditional approaches to OOD detection can be broadly categorized into logit-based \cite{Liu2020EnergybasedOD,hendrycks2022scaling,sun2021react}, feature-based \cite{lee2018simple,saito2020universal,park2023understanding}, probability-based \cite{sun2021react,basart2022scaling,liang2017enhancing,huang2021importance}, and reconstruction-based methods \cite{heng2024out,yang2024diffusion}. Feature‑based methods extract intermediate representations from ID data using a discriminative model and measure distances, such as the Mahalanobis distance, between test samples and the ID feature distribution \cite{denouden2018improving}. Recent variants improve robustness by leveraging self-supervised or pre-trained models for more discriminative features \cite{tack2020csi,sehwag2021ssd}.

%Another line of research focuses on training-time regularization, incorporating auxiliary OOD data or outlier exposure to enhance robustness during model training \cite{yu2019unsupervised,hendrycks2018deep}. However, most of these approaches are designed for single-modal backbones, limiting their generalization capacity in multimodal settings where both visual and textual inputs are involved.

\vspace{0.5em}
\noindent\textbf{Training-Free OOD Detection with Vision-Language Models}.
The advent of vision-language models, particularly CLIP \cite{radford2021learning}, has opened new research frontiers for training-free OOD detection by leveraging powerful pre-trained joint representations. These methods utilize scoring functions to quantify the semantic discrepancy between ID and OOD samples without requiring model fine-tuning.
Early works such as ZOC \cite{esmaeilpour2022zero}, and MCM \cite{ming2022delving} apply CLIP-based embeddings for OOD detection using similarity-based metrics. GL‑MCM~\cite{miyai2025gl} extends this MCM score by incorporating local visual features to enhance OOD detection performance. CLIPN \cite{wang2023clipn} proposes negative text encoders to better seperate OOD samples. DPM \cite{zhang2024vision}  matches domain‑specific visual features with both textual and visual prototypes, improving ID–OOD separability. In addition, Outlier exposure methods like NegLabel \cite{jiang2024negative} and AdaNeg \cite{zhang2024adaneg} leverages a large set of semantically diverse negative labels to enhance separability between ID and OOD samples. CLIP-Scope \cite{fu2025clipscope} mines nearest and farthest WordNet labels for broad OOD coverage and applies a Bayesian posterior update using historical class‑likelihoods to enhance zero‑shot OOD detection. %Meanwhile, OLE \cite{ding2024zero} and EOE \cite{cao2024envisioning} explore synthetic outlier generation and expert-guided knowledge to improve OOD identification—again, without modifying the pre-trained VLM backbone.
\vspace{0.5em}\\
\noindent\textbf{Prompt Learning for OOD Detection}.
Prompt learning has recently emerged as an effective and parameter-efficient paradigm for adapting foundation models to novel tasks under limited supervision. Initially introduced in NLP \cite{petroni2019language}, prompt tuning utlilizes trainable prompt tokens to the input rather than updating the full model. In the vision-language domain, CoOp \cite{zhou2022learning} proposes learning a set of shared context tokens, while CoCoOp \cite{zhou2022conditional} improves adaptability by making prompts conditional on the visual input features. VPT \cite{jia2022visual} further extends this approach by injecting prompts into the visual encoder layers. While this approaches are effective for in-distribution classification, they often struggle in OOD settings, as prompt tuning methods usually optimize for ID accuracy without explicitly addressing semantic shifts in OOD inputs. To address this, LoCoOp \cite{miyai2023loCoOp} regularizes prompt learning using CLIP’s local features as surrogate OOD features. Similarly, LSN \cite{nie2024out} and NegPrompt \cite{li2024learning} incorporate negative prompts to enhance the semantic separation between ID and OOD categories.

%Nevertheless, prompt-based methods often underperform in detecting unknown OOD instances—especially in few-shot or zero-shot regimes—due to their reliance on ID-centric objectives. These limitations highlight a pressing need for prompt learning paradigms that are explicitly designed for OOD detection in low-resource settings.


\section{Additional Experiments}

\begin{figure}[ht]
    \centering
    \makebox[\textwidth]{%
        \begin{subcaptionbox}{\label{fig:img1}}[0.4\linewidth]
            {\centering\includegraphics[width=\linewidth]{images/iNaturalist_sct3.png}}
        \end{subcaptionbox}
        \hspace{2em} % space between the figures
        \begin{subcaptionbox}{\label{fig:img2}}[0.4\linewidth]
            {\centering\includegraphics[width=\linewidth]{images/iNaturalist_subcoop3.png}}
        \end{subcaptionbox}
    }
    \caption{OOD detection performance on the iNaturalist dataset using (a) SCT and (b) SubCoOp (Ours). }
    \label{fig:two_images1}
\end{figure}

\begin{figure}[ht]
    \centering
    \makebox[\textwidth]{%
        \begin{subcaptionbox}{\label{fig:img1}}[0.38\linewidth]
            {\centering\includegraphics[width=\linewidth]{images/SUN_SCT3.png}}
        \end{subcaptionbox}
        \hspace{2em} % adjust spacing between the figures
        \begin{subcaptionbox}{\label{fig:img2}}[0.38\linewidth]
            {\centering\includegraphics[width=\linewidth]{images/SUN_1.0_MCM22.png}}
        \end{subcaptionbox}
    }
    \caption{OOD detection performance on the SUN dataset using (a) SCT and (b) SubCoOp (Ours).}
    \label{fig:two_images2}
\end{figure}


\begin{table*}[h]
\centering
\caption{OOD detection performance analysis with different backbones with ImageNet-1k dataset.}
\label{tab:ood_detection_results21}
\resizebox{0.97\textwidth}{!}{%
\setlength{\tabcolsep}{3.0pt}
\begin{tabular}{l l cc cc cc cc cc}
\toprule
\textbf{Model} & \textbf{Method} &
\multicolumn{2}{c}{\textbf{iNaturalist}} &
\multicolumn{2}{c}{\textbf{SUN}} &
\multicolumn{2}{c}{\textbf{Places}} &
\multicolumn{2}{c}{\textbf{Texture}} &
\multicolumn{2}{c}{\textbf{Avg}} \\
 &  &
FPR95$\downarrow$ & AUROC$\uparrow$ &
FPR95$\downarrow$ & AUROC$\uparrow$ &
FPR95$\downarrow$ & AUROC$\uparrow$ &
FPR95$\downarrow$ & AUROC$\uparrow$ &
FPR95$\downarrow$ & AUROC$\uparrow$ \\
\midrule
\multirow{2}{*}{ViT-B/32} 
 & SCT      & $29.07^{\scriptsize{\pm 3.90}}$& $94.24^{\scriptsize{\pm 0.44}}$ & $35.27^{\scriptsize{\pm 2.87}}$ & $92.47^{\scriptsize{\pm 0.40}}$ & $39.59^{\scriptsize{\pm 2.40}}$ &$90.36^{\scriptsize{\pm 0.42}}$ & $47.13^{\scriptsize{\pm 1.01}}$ & $88.49^{\scriptsize{\pm 0.80}}$ & $37.77^{\scriptsize{\pm 2.55}}$ & $91.39^{\scriptsize{\pm 0.52}}$\\
 & SubCoOp (Ours)  & $27.50^{\scriptsize{\pm 2.24}}$ & $94.63^{\scriptsize{\pm 0.30}}$ & $33.85^{\scriptsize{\pm 0.50}}$ & $92.89^{\scriptsize{\pm 0.27}}$ & $38.46^{\scriptsize{\pm 1.00}}$ & $91.42^{\scriptsize{\pm 0.37}}$ &$47.57^{\scriptsize{\pm 2.29}}$ & $88.77^{\scriptsize{\pm 0.62}}$ & $36.85^{\scriptsize{\pm 1.51}}$ & $91.93^{\scriptsize{\pm 0.39}}$\\
\midrule
\multirow{2}{*}{RN-50}
 & SCT      & 40.33^{\scriptsize{\pm 1.25}} & 91.83^{\scriptsize{\pm 0.12}} & 36.43^{\scriptsize{\pm 1.10}} & 91.65^{\scriptsize{\pm 0.19}} & 43.78^{\scriptsize{\pm 1.36}} & 88.15^{\scriptsize{\pm 0.43}} & 37.62^{\scriptsize{\pm 0.93}} & 90.36^{\scriptsize{\pm 0.16}} & $39.54^{\scriptsize{\pm 1.16}}$ & $90.50^{\scriptsize{\pm 0.23}}$ \\
 & SubCoOp (Ours)  & 40.09^{\scriptsize{\pm 1.08}} & 92.21^{\scriptsize{\pm 0.14}} & 36.12^{\scriptsize{\pm 0.96}} & 91.74^{\scriptsize{\pm 0.22}} & 43.08^{\scriptsize{\pm 1.41}} & 88.63^{\scriptsize{\pm 0.73}} & 37.51^{\scriptsize{\pm 0.53}} & 90.31^{\scriptsize{\pm 0.13}} & $39.20^{\scriptsize{\pm 1.00}}$ & $90.72^{\scriptsize{\pm 0.30}}$\\
\bottomrule
\end{tabular}}
\end{table*}








\begin{table}[h]
\centering
\caption{ID classification accuracy with different baselines(\%) utilizing ImageNet-1k dataset }
\label{tab:id_accuracy}
\begin{tabular}{lc}
\toprule
\textbf{Method} & \textbf{ID Accuracy}  \\
\midrule
\textit{Zero-shot methods} \\
MCM  & 66.7 \\
GL-MCM & 66.7 \\
\midrule
\textit{CLIP-based post-hoc methods} \\
MSP  & 66.7 \\
ODIN  & 66.7 \\
Energy  & 66.7 \\
ReAct   & 66.7 \\
MaxLogit  & 66.7 \\
\midrule
\textit{Prompt tuning based methods} \\
CoOp & 71.93 \\
NegPrompt & 71.93 \\
SCT& 71.72\\
LoCoOp &71.43 \\
IDlike  & 71.04 \\
SubCoOp & 70.57\\



\bottomrule
\end{tabular}
\end{table}


\begin{table*}[h]
\centering
\caption{OOD detection anslysis utilizing ImageNet-1k as ID dataset with varying entropy regularization weights ( $\lambda_3$).}
\label{tab:ood_results2}
\resizebox{0.8\textwidth}{!}{%
\setlength{\tabcolsep}{4pt} 
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Places}} & \multicolumn{2}{c}{\textbf{Texture}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}
& FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\
\midrule

SubCoOP ($\lambda_3$=0)   & 16.20 & 96.67 & 34.36 & 93.60 & 42.19 & 90.09 & 43.19 & 89.43 & 34.00 & 92.45 \\
SubCoOP ($\lambda_3$=0.1) & 12.82 & 97.28 & 18.97 & 95.72 & 29.62 & 92.46 & 41.16 & 90.69 & 25.64 & 94.02 \\
SubCoOP ($\lambda_3$=0.3) &15.31 & 96.59 & 18.16 & 96.35 & 28.89 & 92.67 & 41.03 & 90.61 & 25.85 & 93.98 \\
SubCoOP ($\lambda_3$=0.4) & 15.61 & 96.58 & 19.14 & 95.82 & 29.38 & 92.12 & 40.60 & 90.51 & 25.97 & 93.78 \\
SubCoOP ($\lambda_3$=0.5) & 14.52 & 97.08 & 19.82 & 95.56 & 29.94 & 91.91 & 42.45 & 90.27 & 26.83 & 93.71 \\
SubCoOP ($\lambda_3$=1.0) & 15.08 & 96.71 & 22.01 & 94.89 & 34.00 & 91.19 & 44.22 & 88.91 & 28.83 & 92.93 \\

\bottomrule
\end{tabular}}
\end{table*}



\begin{table}[!t]
\centering
\caption{Comparison of FPR95 and AUROC scores on various OOD datasets with ID dataset ImageNet-1k. All methods use the same CLIP-ViT-B/16 backbone, and 1-shot training setting.}
\label{IMG1k}
\resizebox{1\textwidth}{!}{%

\setlength{\tabcolsep}{3.2pt}
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Places365}} & \multicolumn{2}{c}{\textbf{Textures}} & \multicolumn{2}{c}{\textbf{Average}} \\
 & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\
\midrule

\multicolumn{11}{c}{\textit{Prompt tuning based methods (1-shot)}} \\
CoOp & $27.99^{\scriptsize{\pm 4.18}}$ & $93.73^{\scriptsize{\pm 1.27}}$ & $36.03^{\scriptsize{\pm 4.02}}$ & $90.95^{\scriptsize{\pm 0.57}}$& $45.46^{\scriptsize{\pm 4.26}}$ & $87.82^{\scriptsize{\pm 1.42}}$& $53.70^{\scriptsize{\pm 1.79}}$ & $84.59^{\scriptsize{\pm 0.67}}$&  $40.80^{\scriptsize{\pm 3.56}}$ & $89.77^{\scriptsize{\pm 0.98}}$\\
LoCoOp & $26.81^{\scriptsize{\pm 2.78}}$ & $94.45^{\scriptsize{\pm 0.72}}$ & $26.16^{\scriptsize{\pm 1.13}}$ & $94.06^{\scriptsize{\pm 0.21}}$ & $35.18^{\scriptsize{\pm 1.05}}$ & $91.10^{\scriptsize{\pm 0.13}}$& $50.53^{\scriptsize{\pm 0.33}}$ & $86.96^{\scriptsize{\pm 0.60}}$ & $34.67^{\scriptsize{\pm 1.32}}$ & $91.64^{\scriptsize{\pm 0.42}}$\\
IDLike & $12.07^{\scriptsize{\pm 0.88}}$ & $97.65^{\scriptsize{\pm 0.10}}$ & $40.55^{\scriptsize{\pm 5.84}}$ & $91.07^{\scriptsize{\pm 1.80}}$ & $47.94^{\scriptsize{\pm 5.24}}$ & $88.31^{\scriptsize{\pm 2.05}}$ & $38.34^{\scriptsize{\pm 13.39}}$ & $89.67^{\scriptsize{\pm 4.03}}$ & $34.72^{\scriptsize{\pm 0.80}}$ & $91.67^{\scriptsize{\pm 0.07}}$ \\
NegPrompt & $65.03^{\scriptsize{\pm 8.69}}$ & $84.56^{\scriptsize{\pm 2.52}}$ & $44.39^{\scriptsize{\pm 1.66}}$ & $89.63^{\scriptsize{\pm 0.66}}$ & $51.31^{\scriptsize{\pm 6.21}}$ & $86.55^{\scriptsize{\pm 2.19}}$ & $63.76^{\scriptsize{\pm 3.02}}$ & $83.76^{\scriptsize{\pm 3.02}}$ & $62.08^{\scriptsize{\pm 3.71}}$ & $81.13^{\scriptsize{\pm 1.78}}$ \\
LSN & $59.28^{\scriptsize{\pm 7.02}}$ & $87.20^{\scriptsize{\pm 3.15}}$ & $40.15^{\scriptsize{\pm 0.82}}$ & $91.47^{\scriptsize{\pm 0.14}}$ & $46.11^{\scriptsize{\pm 1.86}}$ & $88.74^{\scriptsize{\pm 0.57}}$ & $60.34^{\scriptsize{\pm 0.14}}$ & $88.92^{\scriptsize{\pm 0.42}}$ & $51.47^{\scriptsize{\pm 1.53}}$ & $87.84^{\scriptsize{\pm 0.58}}$ \\
SCT   & $20.77^{\scriptsize{\pm4.12}}$ & $95.15^{\scriptsize{\pm1.15}}$
& $24.92^{\scriptsize{\pm2.03}}$ & $94.17^{\scriptsize{\pm0.53}}$& $33.35^{\scriptsize{\pm2.03}}$ & $91.08^{\scriptsize{\pm0.49}}$ & $50.28^{\scriptsize{\pm1.18}}$ & $85.71^{\scriptsize{\pm0.08}}$& $32.83^{\scriptsize{\pm2.34}}$ & $91.53^{\scriptsize{\pm0.56}}$\\
\textbf{SubCoOp} & $20.44^{\scriptsize{\pm4.71}}$ & $94.96^{\scriptsize{\pm1.01}}$ & $24.13^{\scriptsize{\pm3.60}}$ & $94.36^{\scriptsize{\pm0.92}}$ & $32.45^{\scriptsize{\pm3.02}}$ & $91.78^{\scriptsize{\pm0.72}}$ & $50.07^{\scriptsize{\pm1.11}}$ & $87.15^{\scriptsize{\pm0.08}}$ & $31.96^{\scriptsize{\pm 3.11}}$ & $91.83^{\scriptsize{\pm 0.68}}$ \\
\hline
\textbf{CoOp-SR} & $23.87^{\scriptsize{\pm 4.49}}$ & $94.88^{\scriptsize{\pm 1.32}}$ & $34.68^{\scriptsize{\pm 1.65}}$ & $90.72^{\scriptsize{\pm 0.74}}$& $42.86^{\scriptsize{\pm 1.14}}$ & $88.92^{\scriptsize{\pm 0.71}}$ & $51.83^{\scriptsize{\pm 1.67}}$ & $84.25^{\scriptsize{\pm 0.31}}$ & $38.31^{\scriptsize{\pm 2.24}}$ & $89.69^{\scriptsize{\pm 0.77}}$\\
\textbf{LoCoOp-SR} & $26.31^{\scriptsize{\pm 7.74}}$ & $94.47^{\scriptsize{\pm 1.43}}$ & $26.13^{\scriptsize{\pm 1.89}}$ & $94.41^{\scriptsize{\pm 0.23}}$& $34.85^{\scriptsize{\pm 1.14}}$ & $91.26^{\scriptsize{\pm 0.28}}$ & $50.62^{\scriptsize{\pm 1.67}}$ & $87.01^{\scriptsize{\pm 0.31}}$ & $34.48^{\scriptsize{\pm 3.11}}$ & $91.79^{\scriptsize{\pm 0.56}}$\\

\bottomrule
\end{tabular}}
\end{table}



\begin{table*}[h]
\centering
\caption{Comparison of FPR95 and AUROC scores using different few-shot techniques (\%) on various OOD datasets with ID dataset ImageNet-1k.}
\label{tab:ood_results22}
\resizebox{1\textwidth}{!}{%
\setlength{\tabcolsep}{4pt} 
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Places}} & \multicolumn{2}{c}{\textbf{Texture}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}
& FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\
\midrule

SCT (1-shot)  & $20.77^{\scriptsize{\pm4.12}}$ & $95.15^{\scriptsize{\pm1.15}}$
& $24.92^{\scriptsize{\pm2.03}}$ & $94.17^{\scriptsize{\pm0.53}}$& $33.35^{\scriptsize{\pm2.03}}$ & $91.08^{\scriptsize{\pm0.49}}$ & $50.28^{\scriptsize{\pm1.18}}$ & $85.71^{\scriptsize{\pm0.08}}$& $32.83^{\scriptsize{\pm2.34}}$ & $91.53^{\scriptsize{\pm0.56}}$\\
SCT (4-shot) & $22.78^{\scriptsize{\pm1.06}}$ & $95.01^{\scriptsize{\pm0.56}}$ & $22.97^{\scriptsize{\pm0.72}}$ & $95.16^{\scriptsize{\pm0.41}}$ & $33.10^{\scriptsize{\pm2.01}}$ & $91.80^{\scriptsize{\pm0.43}}$ & $44.68^{\scriptsize{\pm2.22}}$ & $89.12^{\scriptsize{\pm0.68}}$ & $30.88^{\scriptsize{\pm1.50}}$ & $92.77^{\scriptsize{\pm0.52}}$   \\
SCT (8-shot) & $17.45^{\scriptsize{\pm1.19}}$ & $96.50^{\scriptsize{\pm0.20}}$ & $24.23^{\scriptsize{\pm0.23}}$ & $94.82^{\scriptsize{\pm0.31}}$ & $33.90^{\scriptsize{\pm0.58}}$ & $91.69^{\scriptsize{\pm0.19}}$ & $46.71^{\scriptsize{\pm2.09}}$ & $88.74^{\scriptsize{\pm0.67}}$ & $30.57^{\scriptsize{\pm1.02}}$ & $92.94^{\scriptsize{\pm0.34}}$\\
SCT (16-shot) & $16.14^{\scriptsize{\pm 1.81}}$ & $96.68^{\scriptsize{\pm 0.29}}$ & $21.57^{\scriptsize{\pm 1.20}}$ & $95.23^{\scriptsize{\pm 0.26}}$ & $31.47^{\scriptsize{\pm 0.89}}$ & $91.89^{\scriptsize{\pm 0.25}}$ & $43.75^{\scriptsize{\pm 0.56}}$ & $88.83^{\scriptsize{\pm 0.45}}$ & $28.23^{\scriptsize{\pm 1.12}}$ & $93.16^{\scriptsize{\pm 0.31}}$\\
SubCoOp (1-shot)  & $20.44^{\scriptsize{\pm4.71}}$ & $94.96^{\scriptsize{\pm1.01}}$ & $24.13^{\scriptsize{\pm3.60}}$ & $94.36^{\scriptsize{\pm0.92}}$ & $32.45^{\scriptsize{\pm3.02}}$ & $91.78^{\scriptsize{\pm0.72}}$ & $50.07^{\scriptsize{\pm1.11}}$ & $87.15^{\scriptsize{\pm0.08}}$ & $31.96^{\scriptsize{\pm 3.11}}$ & $91.83^{\scriptsize{\pm 0.68}}$ \\
SubCoOp (4-shot) & $16.66^{\scriptsize{\pm2.58}}$ & $96.55^{\scriptsize{\pm0.43}}$& $20.65^{\scriptsize{\pm2.06}}$ & $95.63^{\scriptsize{\pm0.57}}$& $29.79^{\scriptsize{\pm0.91}}$ & $92.54^{\scriptsize{\pm0.23}}$ & $45.16^{\scriptsize{\pm1.68}}$ & $89.23^{\scriptsize{\pm0.69}}$
& $28.05^{\scriptsize{\pm1.81}}$ & $93.50^{\scriptsize{\pm0.48}}$ \\
SubCoOp (8-shot) & $15.45^{\scriptsize{\pm2.62}}$ & $96.64^{\scriptsize{\pm0.32}}$ & $18.47^{\scriptsize{\pm0.34}}$ & $96.18^{\scriptsize{\pm0.07}}$ & $27.28^{\scriptsize{\pm4.91}}$ & $93.26^{\scriptsize{\pm1.62}}$ & $43.22^{\scriptsize{\pm1.22}}$ & $89.86^{\scriptsize{\pm0.14}}$ & $26.11^{\scriptsize{\pm 2.27}}$ & $93.49^{\scriptsize{\pm 0.54}}$\\
SubCoOp (16-shot) & $14.02^{\scriptsize{\pm 1.56}}$ & $97.02^{\scriptsize{\pm 0.39}}$ & $19.06^{\scriptsize{\pm 1.21}}$ & $95.79^{\scriptsize{\pm 0.34}}$ & $30.14^{\scriptsize{\pm 1.93}}$ & $92.35^{\scriptsize{\pm 0.49}}$ & $41.08^{\scriptsize{\pm 1.00}}$ & $90.65^{\scriptsize{\pm 0.24}}$ & $26.08^{\scriptsize{\pm 1.43}}$ & $93.95^{\scriptsize{\pm 0.37}}$\\
\bottomrule
\end{tabular}}
\end{table*}



Figures~\ref{fig:two_images1} and~\ref{fig:two_images2} show ID/OOD histograms for iNaturalist and SUN, comparing SCT with SubCoOp. SubCoOp provides better separation between ID and OOD distributions, with reduced overlap in plots (b), highlighting its stronger capability to discriminate OOD samples.
%Figure~\ref{fig:four_individual_captions} presents histograms of GL‑MCM OOD detection scores for SubCoOp across four OOD datasets with ImageNet‑1k as ID.
This minimal overlap between ID and OOD distributions demonstrates the strong separability achieved by our subspace regularization.

Table \ref{tab:ood_results22} compares the OOD detection performance of SCT and SubCoOp under varying few-shot settings  using ImageNet-1k as the ID data set. Both methods demonstrate consistent improvements in FPR95 and AUROC as the number of shots increases. SubCoOp demonstrates a substantial performance gain over SCT, especially in higher-shot settings, achieving lower average FPR95 and higher average AUROC. In the 8‑shot setting, SubCoOp consistently outperforms SCT across all OOD datasets, reducing average FPR95 from 30.57\% to 26.11\% and improving AUROC from 92.94\% to 93.49\%.
Notable gains include substantial FPR95 reductions on SUN of 5.76\% and Texture of 7.35\%, highlighting SubCoOp’s superior OOD separability when more labeled examples are available.

Table \ref{tab:ood_detection_results21} presents OOD detection results across four OOD datasets for two backbone architectures, ViT-B/32 and RN-50, comparing SCT with SubCoOp.
We present the ID classification performance of different methods in Table ~\ref{tab:id_accuracy}. Zero-shot and post-hoc methods achieve 66.7\% ID accuracy on ImageNet-1k, whereas prompt-tuning approaches such as CoOp and NegPrompt improve this to approximately 71.92\%. On the other hand, IDLike and LoCoOp attain 71.04\% and 71.43\% ID accuracy, respectively. Our proposed SubCoOp achieves a comparable 70.57\% ID accuracy while delivering the best overall OOD detection performance.\\Table \ref{tab:ood_results2} presents the effect of varying the entropy regularization weight ($\lambda_3$) on OOD detection performance for SubCoOp.
It is evident that moderate values of $\lambda_3$  between 0.2 and 0.3 consistently obtain the best trade‑off between FPR95 and AUROC across all four OOD datasets.
For instance, $\lambda_3$=0.2 achieves the lowest average FPR95 of 25.64\% with a corresponding AUROC of 94.02\%, while $\lambda_3$=0.3 delivers a comparable FPR95 of 25.85\% but slightly higher AUROC of 93.98\%.
Extremely low value $\lambda_3$=0 or high value $\lambda_3$=1.0 results in degraded performance.\\
Table~\ref{IMG1k} reports the OOD detection performance of various methods on ImageNet-1k under the 1-shot setting using the CLIP-ViT/B-16 backbone. Among prompt-tuning approaches, SubCoOp achieves the lowest FPR95 of 32.18\% and the highest  AUROC of 91.83\%, outperforming the other state-of-the-art baselines across most OOD datasets. The SR-enhanced variants, CoOp-SR and LoCoOp-SR, improve OOD separability compared to their respective baselines. Specifically, CoOp-SR reduces the average FPR95 from 40.80\% for CoOp to 38.31\% while maintaining a high AUROC of 89.69\% compared to 89.77\% for CoOp.  These results demonstrate that SubCoOp and SR-based enhancements offer consistent gains in few-shot OOD detection over standard prompt-tuning baselines. 
\\Table \ref{tab:ood_results3} presents the OOD detection performance of CoOp, LoCoOp, SCT, and the proposed SubCoOp on ImageNet‑100 as ID data.
SubCoOp achieves the best overall results, with the lowest average FPR95 of 11.60\% and the highest average AUROC of 97.80\%, consistently outperforming the other methods across all four OOD datasets. While SCT also delivers strong results with FPR95 12.50\% and AUROC 97.25\%, SubCoOp offers further gains, demonstrating its robustness and effectiveness in few‑shot OOD detection.\\
\\
\\
\quad
\begin{table*}[h]
\centering
\caption{Comparison of FPR95 and AUROC scores (\%) on various OOD datasets with ID dataset ImageNet-100. }
\label{tab:ood_results3}
\resizebox{1\textwidth}{!}{%
\setlength{\tabcolsep}{4pt} 
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{iNaturalist}} & \multicolumn{2}{c}{\textbf{SUN}} & \multicolumn{2}{c}{\textbf{Places}} & \multicolumn{2}{c}{\textbf{Texture}} & \multicolumn{2}{c}{\textbf{Average}} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}
& FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ \\
\midrule
%LSN & $3.54^{\scriptsize{\pm0.31}}$ & $98.90^{\scriptsize{\pm0.09}}$ & $9.11^{\scriptsize{\pm0.87}}$ & $98.04^{\scriptsize{\pm0.17}}$ & $13.01^{\scriptsize{\pm0.50}}$ & $97.15^{\scriptsize{\pm0.11}}$ & $12.43^{\scriptsize{\pm0.21}}$ & $97.88^{\scriptsize{\pm0.12}}$ & $9.52^{\scriptsize{\pm4.02}}$ & $97.99^{\scriptsize{\pm0.71}}$ \\

CoOp & $23.70^{\scriptsize{\pm6.29}}$ & $96.67^{\scriptsize{\pm0.57}}$ & $21.30^{\scriptsize{\pm6.00}}$ & $96.53^{\scriptsize{\pm0.51}}$ & $25.75^{\scriptsize{\pm2.37}}$ & $95.28^{\scriptsize{\pm0.42}}$ & $19.39^{\scriptsize{\pm1.27}}$ & $96.85^{\scriptsize{\pm0.16}}$ & $22.54^{\scriptsize{\pm 3.98}}$ & $96.33^{\scriptsize{\pm 0.42}}$\\
LoCoOp & $11.30^{\scriptsize{\pm10.01}}$ & $97.99^{\scriptsize{\pm0.46}}$ & $13.90^{\scriptsize{\pm7.35}}$ & $96.92^{\scriptsize{\pm0.29}}$ & $20.57^{\scriptsize{\pm10.13}}$ & $95.50^{\scriptsize{\pm0.39}}$ & $17.23^{\scriptsize{\pm8.56}}$ & $96.16^{\scriptsize{\pm0.52}}$ & 
$15.75^{\scriptsize{\pm 9.01}}$ & $96.64^{\scriptsize{\pm 0.42}}$\\
SCT & $5.26^{\scriptsize{\pm0.21}}$ & $98.71^{\scriptsize{\pm0.35}}$ & $11.21^{\scriptsize{\pm3.20}}$ & $97.54^{\scriptsize{\pm1.16}}$ & $16.21^{\scriptsize{\pm4.12}}$ & $96.47^{\scriptsize{\pm0.78}}$ & $17.32^{\scriptsize{\pm1.76}}$ & $96.29^{\scriptsize{\pm0.63}}$ & $12.50^{\scriptsize{\pm4.32}}$ & $97.25^{\scriptsize{\pm0.81}}$ \\
\bottomrule
SubCoOp & $5.03^{\scriptsize{\pm1.93}}$ & $98.83^{\scriptsize{\pm0.28}}$
& $9.70^{\scriptsize{\pm0.98}}$ & $98.03^{\scriptsize{\pm0.23}}$ & $15.06^{\scriptsize{\pm0.32}}$ & $96.73^{\scriptsize{\pm0.07}}$ &
$16.59^{\scriptsize{\pm0.58}}$ & $97.59^{\scriptsize{\pm0.31}}$ &
$11.60^{\scriptsize{\pm 0.95}}$ & $97.80^{\scriptsize{\pm 0.22}}$\\
\bottomrule
\end{tabular}}
\end{table*}
\end{comment}
